A stable partitioned FSI algorithm for rigid bodies and incompressible flow in three dimensions

This paper describes a novel partitioned algorithm for fluid-structure interaction (FSI) problems that couples the motion of rigid bodies and incompressible flow. This is the first partitioned algorithm that remains stable and second-order accurate, without sub-time-step iterations, for very light, and even zero-mass, bodies in three dimensions. This new added-mass partitioned (AMP) algorithm extends the previous developments in [1, 2] by generalizing the added-damping tensors to account for arbitrary three-dimensional rotations, and by employing a general quadrature for the surface integral over a rigid body to derive the discrete AMP interface condition for the fluid pressure. Stability analyses for two three-dimensional model problems show that the algorithm remains stable for bodies of any mass when applied to the relevant model problems. The resulting AMP algorithm is implemented in parallel using a moving composite grid framework to treat one or more rigid bodies in complex three-dimensional configurations. The new three-dimensional algorithm is verified and validated though several benchmark problems, including the motion of a sphere in a viscous incompressible fluid and the interaction of a bi-leaflet mechanical heart valve and a pulsating fluid. Numerical simulations confirm the predictions of the stability analysis even for complex problems, and show that the AMP algorithm remains stable, without sub-iterations, for light and even zero-mass three-dimensional rigid bodies of general shape. These benchmark problems are further used to examine the parallel performance of the algorithm and to investigate the conditioning of the linear system for the pressure including the newly derived AMP interface conditions.

==> texFiles/heartValve3Dspeed.tex <==
{% ------ STREAMLINES ------
\newcommand{\drawContour}[7]{%
%
%
\begin{scope}[#1]
\draw(0.0,0) node[anchor=south west,xshift=-4pt,yshift=+0pt] {\trimfig{heartValve/3d/#2}{\figWidth}};
  \draw(.7,4.75) node[draw,fill=white,anchor=west,xshift=2pt,yshift=-1pt] {\scriptsize #5};
 % colour bar:
\begin{scope}[xshift=5pt,yshift=-2pt]
  \draw (\xcb,\ycb) node[anchor=south west,xshift=0.cm,yshift=.5cm,rotate=-90] {\trimfigcb{fig/colourBarLines}{\cbWidth}{\cbHeight}};
  \draw (.8,0) node[anchor=north,xshift=+3pt,yshift=+2pt] {\scriptsize $#6$};
  \draw (3.7,0) node[anchor=north,xshift=+0pt,yshift=+2pt] {\scriptsize $#7$};
\end{scope}
\end{scope}
}
% -- for colour bar ----
\newcommand{\cbWidth}{.2cm}% colour bar width
\newcommand{\cbHeight}{3.3cm}% colour bar height
\newcommand{\xcb}{.5cm}% colour bar lower left corner
\newcommand{\ycb}{-.2cm}% colour bar lower left corner
\setlength{\ycbTop}{\ycb+\cbHeight}% colour bar top label position
\setlength{\ycbMid}{\ycb+\cbHeight*\real{.5}}% colour bar top label position
\newcommand{\trimfigcb}[3]{\includegraphics[width=#2, height=#3, clip, trim=17cm 2.35cm 1.65cm 2.35cm]{#1}}
%
% ============================ DRAW ===================================
\newcommand{\figWidth}{4.2cm}
\newcommand{\trimfig}[2]{\trimw{#1}{#2}{.2}{.2}{.1}{.35}}
\newcommand{\figWidtha}{4.25cm}
\newcommand{\trimfiga}[2]{\trimFig{#1}{#2}{.57}{.425}{.0}{.17}}
\begin{figure}[htb]
\begin{center}
%\resizebox{16cm}{!}{% START resize box
\begin{tikzpicture}[scale=1]
  \useasboundingbox (0.0,.25) rectangle (16.,11.2);  % set the bounding box (so we have less surrounding white space)
% 
%  top row: 
\begin{scope}[yshift=6cm]
 \drawContour{xshift=-0.5cm,yshift=0.0cm}{heartValve3dt0p2speed}{$p$}{$p$}{$t=0.2$}{0.0}{1.26};
 \drawContour{xshift= 3.5cm,yshift=0.0cm}{heartValve3dt0p5speed}{$p$}{$p$}{$t=0.5$}{0.0}{4.00};
 \drawContour{xshift= 7.5cm,yshift=0.0cm}{heartValve3dt0p8speed}{$p$}{$p$}{$t=0.8$}{0.0}{5.43};
 \drawContour{xshift=11.5cm,yshift=0.0cm}{heartValve3dt1p0speed}{$p$}{$p$}{$t=1.0$}{0.0}{4.46};
\end{scope}
%  bottom row: 
 \drawContour{xshift=-0.5cm,yshift=0.0cm}{heartValve3dt1p1speed}{$p$}{$p$}{$t=1.1$}{0.0}{2.99};
 \drawContour{xshift= 3.5cm,yshift=0.0cm}{heartValve3dt1p5speed}{$p$}{$p$}{$t=1.5$}{0.0}{3.96};
 \drawContour{xshift= 7.5cm,yshift=0.0cm}{heartValve3dt1p6speed}{$p$}{$p$}{$t=1.6$}{0.0}{3.83};
 \drawContour{xshift=11.5cm,yshift=0.0cm}{heartValve3dt2p0speed}{$p$}{$p$}{$t=2.0$}{0.0}{3.73};
% 
% ---------------
% grid:
%\draw[step=1cm,gray] (0,0) grid (16,11.2);
\end{tikzpicture}
%}% end resize box
\end{center}
  \caption{Mechanical heart valve in 3D. Computed flow speed at selected times using the composite grid $\Gchv^{(1)}$.  
}
  \label{fig:heartValve3Dstreamlines}
\end{figure}
}

